The Jodrell Bank Glitch Catalogue: 106 new rotational glitches in 70 pulsars

Pulsar glitches are rapid spin-up events that occur in the rotation of neutron stars, providing a valuable probe into the physics of the interiors of these objects. Long-term monitoring of a large number of pulsars facilitates the detection of glitches and the robust measurements of their parameters. The Jodrell Bank pulsar timing programme regularly monitors more than 800 radio pulsars and has accrued, in some cases, over 50 years of timing history on individual objects. In this paper we present 106 new glitches in 70 radio pulsars as observed up to the end of 2018. For 70% of these pulsars, the event we report is its only known glitch. For each new glitch we provide measurements of its epoch, amplitude and any detected changes to the spin-down rate of the star. Combining these new glitches with those listed in the Jodrell Bank glitch catalogue we analyse a total sample of 543 glitches in 178 pulsars. We model the distribution of glitch amplitudes and spin-down rate changes using a mixture of two Gaussian components. We corroborate the known dependence of glitch rate and activity on pulsar spin-down rates and characteristic ages, and show that younger pulsars tend to exhibit larger glitches. Pulsars whose spin-down rates between $10^{-14}$ Hz s$^{-1}$ and $10^{-10.5}$ Hz s$^{-1}$ show a mean reversal of 1.8% of their spin-down as a consequence of glitches. Our results are qualitatively consistent with the superfluid vortex unpinning models of pulsar glitches.

==> glitch.tab.tex <==
\begin{longtable}[]{@{}lllllllll@{}}
\toprule
\hline \hline
Name & J-Name & Epoch (MJD) & GLEP err & $\frac{\Delta \nu}{\nu}\times 10^{-9}$ & dF0/F0 err (e-9) & $\frac{\Delta \Dot{\nu}}{\Dot{\nu}} \times 10^{-3}$ & dF1/F1err(e-3) & Reference\tabularnewline
\midrule \hline \hline
\endhead 
B0154+61 & 0157+6212 & 58299 & 4 & 2.64 & 0.12 & X & X & New -
bshaw\tabularnewline
J0205+6449 & 0205+6449 & 54907 & 3 & 1733 & 6 & 6 & 1 & New - Our
measurement\tabularnewline
J0205+6449 & 0205+6449 & 55275 & 1 & 3.8 & 0.2 & -0.92 & 0.02 & New -
bshaw\tabularnewline
J0205+6449 & 0205+6449 & 55350.3 & 0.7 & 6.9 & 0.3 & -0.54 & 0.04 & New
- bshaw\tabularnewline
J0205+6449 & 0205+6449 & 55416 & 1 & 4.9 & 0.4 & -0.76 & 0.04 & New -
bshaw\tabularnewline
J0205+6449 & 0205+6449 & 55461 & 1 & 6.9 & 0.5 & X & X & bshaw - not
sure about this one\tabularnewline
J0205+6449 & 0205+6449 & 55511 & 2 & 10.6 & 0.8 & 0.6 & 0.2 & New -
bshaw\tabularnewline
J0205+6449 & 0205+6449 & 55721.56 & 0.13 & 118.8 & 10.7 & 2.65 & 0.06 &
New - Our measurement\tabularnewline
J0205+6449 & 0205+6449 & 55816 & 8 & 3005 & 40 & 18.8 & 0.3 & New - Our
measurement\tabularnewline
J0205+6449 & 0205+6449 & 56835 & 24 & 87 & 11 & 2.6 & 0.2 & New - Our
measurement\tabularnewline
J0205+6449 & 0205+6449 & 57358 & 1 & 531 & 4 & 6 & 1 & New - agl (mjk's
measurement)\tabularnewline
J0205+6449 & 0205+6449 & 57697 & 1 & 41.9 & 1.4 & X & X & New - agl
(mjk's measurement)\tabularnewline
J0205+6449 & 0205+6449 & 58321 & 99 & 3162 & 3 & 20.4 & 0.1 & New - agl
(bshaw measurement)\tabularnewline
J0215+6218 & 0215+6218 & 55945 & 5 & 0.1 & 0.01 & 0.6 & 0.2 & New - Our
measurement\tabularnewline
%B0355+54 & 0358+5413 & 51679 & 15 & 0.06 & 0.04 & 0 & 0.2 &
%Espinoza+2011 {[}\textless a
%href="http://adsabs.harvard.edu/abs/2011MNRAS.414.1679E"\textgreater elsk11\textless/a\textgreater{]}\tabularnewline
%B0355+54 & 0358+5413 & 51969 & 1 & 0.7 & 0.2 & 15 & 7 & Espinoza+2011
%{[}\textless a
%href="http://adsabs.harvard.edu/abs/2011MNRAS.414.1679E"\textgreater elsk11\textless/a\textgreater{]}\tabularnewline
%B0355+54 & 0358+5413 & 52943 & 3 & 2 & 1 & -39 & 76 & Espinoza+2011
%{[}\textless a
%href="http://adsabs.harvard.edu/abs/2011MNRAS.414.1679E"\textgreater elsk11\textless/a\textgreater{]}\tabularnewline
%B0355+54 & 0358+5413 & 53209 & 2 & 1 & 1 & 207 & 70 & Espinoza+2011
%{[}\textless a
%href="http://adsabs.harvard.edu/abs/2011MNRAS.414.1679E"\textgreater elsk11\textless/a\textgreater{]}\tabularnewline
B0410+69 & 0410+69 & 57207 & 58 & 0.012 & 0.004 & X & X & New - Our
measurement (bshaw)\tabularnewline
B0417+35 & 0417+35 & 57053.6 & 0.1 & 24.63 & 0.03 & 3.6 & X & New - Our
measurement (bshaw)\tabularnewline
B0523+11 & 0525+1115 & 56009 & 3 & 0.27 & 0.03 & X & X & New - Our
measurement\tabularnewline
B0531+21 & 0534+2200 & 55875.5 & 0.1 & 49.2 & 0.3 & X & X & New - Our
measurement\tabularnewline
B0531+21 & 0534+2200 & 57839.92 & 0.06 & 2.14 & 0.11 & 0.27 & 0.03 & New
- Our measurement\tabularnewline
B0531+21 & 0534+2200 & 58470.939 & 0.006 & 2.36 & 0.04 & 0.36 & 0.05 &
New - bshaw\tabularnewline
B0559-05 & 0601-0527 & 54329 & 1 & 0.061 & 0.004 & 0.12 & 0.04 & New -
Our measurement\tabularnewline
J0611+1436 & 0611+1436 & 55818.8 & 0.01 & 5578.29 & 0.24 & 0 & 0 & New -
Our measurement (bshaw - values)\tabularnewline
J0625+1015 & 0625+1015 & 55143 & 10 & 29.5 & 0.2 & 0 & 0 & New - Our
measurement (bshaw)\tabularnewline
J0625+1015 & 0625+1015 & 57660 & 5 & 1.12 & 0.07 & 0 & 0 & New - Our
measurement (bshaw)\tabularnewline
J0631+1036 & 0631+1036 & 55118.83 & 0.01 & 11 & 0.1 & 1.3 & 0.1 & New -
Our measurement\tabularnewline
J0631+1036 & 0631+1036 & 55278.24 & 0.04 & 7 & 0.2 & 2.8 & 0.2 & New -
Our measurement\tabularnewline
J0631+1036 & 0631+1036 & 55702 & 3 & 3280 & 1 & X & X & New - Our
measurement\tabularnewline
J0631+1036 & 0631+1036 & 58341.7 & 0.2 & 27.3 & 0.8 & X & X & New - Our
measurement\tabularnewline
J0631+1036 & 0631+1036 & 58352.14 & 0.04 & 96.7 & 1.5 & X & X & New -
Our measurement\tabularnewline
B0740-28 & 0740-28 & 55210 & 75 & X & X & X & X & new caj (in obs gap).-
cme: can't see it\tabularnewline
B0740-28 & 0742-2822 & 56727.7 & 0.1 & 1.9 & 0.05 & 0.5 & 0.1 & New -
Our measurement; \cite{Basu+2019}\tabularnewline
B0740-28 & 0742-2822 & 58882 & 8 & 2 & 0.4 & X & X & New -
bshaw\tabularnewline
J0818-13 & J0818-13 & 58079 & X & X & X & X & X & New (possible) -
bshaw\tabularnewline
B0844-35 & 0846-3533 & 55665.4 & 0.3 & 0.74 & 0.04 & 3 & 1 & New - Our
measurement\tabularnewline
B0853-33 & 0855-3331 & 54521 & 18 & 0.06 & 0.01 & 0.03 & 0.01 & New -
Our measurement\tabularnewline
B0919+06 & 0922+0638 & 55152 & 6 & 1257 & 1 & X & X & New - Our
measurement\tabularnewline
J1437-6146 & 1437-6146 & 51614 & X & X & X & X & X & pks\tabularnewline
J1635-2614 & 1635-2614 & 56481 & 1 & 0.71 & 0.04 & 0.3 & 0.2 & New - Our
measurement\tabularnewline
J1705-3423 & 1705-3423 & 55503 & 1 & 0.6 & 0.1 & 5 & 1 & New - Our
measurement\tabularnewline
B1706-16 & 1709-1640 & 57592.3 & 0.5 & 0.373 & 0.002 & 0 & 0 & New -
bshaw\tabularnewline
J1726-3530 & 1726-3530 & 57569 & 5 & 14 & 2 & X & X & New -
bshaw\tabularnewline
B1727-33 & 1730-3350 & 55930 & 4 & 2250 & 2 & 7.1 & 0.1 & New - Our
measurement\tabularnewline
B1727-33 & 1730-3350 & 58398 & 1 & 5.9 & 0.5 & X & X & New -
bshaw\tabularnewline
J1730-3353 & 1730-3353 & 54004 & 1 & 68.9 & 0.7 & X & X & New - agl
(bshaw values)\tabularnewline
J1734-3333 & 1734-3333 & 56344.4 & 0.5 & 103 & 8 & 1 & 1 & New (found by
Ryan Shannon) - Our measurement\tabularnewline
J1734-3333 & 1734-3333 & 59012 & 95 & 19 & 10 & X & X & New -
bshaw\tabularnewline
B1737-30 & 1740-3015 & 55213 & 34 & 2668 & 2 & 1.3 & 0.1 & New - Our
measurement; \cite{Yu+2012}\tabularnewline
B1737-30 & 1740-3015 & 55936.2 & 0.1 & 18.6 & 0.1 & 0.2 & 0.1 & New- Our
measurement\tabularnewline
B1737-30 & 1740-3015 & 57468.59 & 0.4 & 229 & 2 & 0 & 0 & New - our
measurement; also Jankowski+2016\tabularnewline
B1737-30 & 1740-3015 & 58240.781 & 0.005 & 837.88 & 0.28 & 1.63 & 0.14 &
New - our measurement; \cite{Basu+2019}\tabularnewline
J1737-3102 & 1737-3102 & 57100.1 & 0.5 & 2.718 & 0.005 & 7.02 & 0.05 &
New - Our Measurement (bshaw)\tabularnewline
J1737-3137 & 1737-3137 & 57116 & 3 & 6.7 & 0.2 & 0 & X & New - Our
measurement (bshaw)\tabularnewline
J1737-3137 & 1737-3137 & 58147 & 43 & 4500 & 1000 & X & X & New - Our
measurement (bshaw)\tabularnewline
J1737-3137 & 1737-3137 & 58858.8 & 0.2 & 1.53 & 0.07 & 0.5 & 0.18 & New
- Our measurement (bshaw)\tabularnewline
J1740+1000 & 1740+1000 & 56160 & 3 & 2917 & 2 & 38 & 4 & New - Our
measurement\tabularnewline
J1746-2856 & 1746-2856 & 57045 & 2 & 24.4 & 0.2 & 2.9 & 0.2 & New - agl
(bshaw values)\tabularnewline
J1751-3323 & 1751-3323 & 57025 & 4 & 12.6 & 0.6 & 0 & 0 & New - Our
measurement (bshaw)\tabularnewline
B1754-24 & 1757-2421 & 55716 & 12 & 7800 & 1 & 27 & 1 & New - Our
measurement\tabularnewline
J1755-0903 & J1755-0903 & 57630 & 3 & 0.85 & 0.05 & -6 & 1 & New -
bshaw\tabularnewline
B1757-24 & 1757-24 & 56949.69 & 0.02 & 2407.8 & 0.4 & 5.67 & 0.05 & New
- cme (bshaw values)\tabularnewline
B1757-24 & 1757-24 & 58566 & 16 & X & X & X & X & New -
bshaw\tabularnewline
B1758-23 & 1801-2304 & 55357.1 & 0.2 & 2 & 1 & -1 & 1 & New - Our
measurement; \cite{Yu+2012} \tabularnewline
B1758-23 & 1801-2304 & 55851.7 & 0.5 & 1.5 & 0.1 & 0.35 & 0.02 & New -
Our measurement\tabularnewline
B1758-23 & 1801-2304 & 56158.36 & 0.002 & 513.9 & 0.2 & 1.4 & 0.1 & New
- Our measurement\tabularnewline
B1758-23 & 1801-2304 & 57586.04 & 0.1 & 96.1 & 0.1 & 0.19 & 0.17 & New -
Our measurement (bshaw)\tabularnewline
B1758-23 & 1801-2304 & 58846 & 6 & 5 & 0.6 & X & X & New - Our
measurement (bshaw)\tabularnewline
B1758-23 & 1801-2304 & 58957 & 2 & 392 & 17 & X & X & New - Our
measurement (bshaw)\tabularnewline
J1759-2922 & 1759-2922 & 54535 & 61 & 0.046 & 0.004 & 0 & 0 & New - Our
measurement (bshaw)\tabularnewline
B1800-21 & 1803-2137 & 55775 & 2 & 4793 & 3 & 18.6 & 0.3 & New - Our
measurement\tabularnewline
B1800-21 & 1803-2137 & 58937 & 5 & 27.11 & 0.23 & 9 & 0.6 & New -
bshaw\tabularnewline
J1809-0119 & 1809-0119 & 55406 & 2 & 1.7 & 0.3 & 0 & 6 & Our
measurement\tabularnewline
J1809-0119 & 1809-0119 & 55803 & 1 & 3 & 0.4 & 0 & 13 & Our
measurement\tabularnewline
J1809-2004 & 1809-2004 & 56229.2 & 0.1 & 48.4 & 0.2 & 1 & 1 & New - Our
measurement\tabularnewline
J1814-1744 & 1814-1744 & 54768.4 & 0.4 & 17 & 1 & 2 & 1 & New - Our
measurement\tabularnewline
J1814-1744 & 1814-1744 & 55626.08 & 0.98 & 15 & 2 & -2 & 2 & New - Our
measurement\tabularnewline
J1821-1419 & 1821-1419 & 53074 & 546 & 225 & 4 & X & X & New - Our
measurement\tabularnewline
J1821-1419 & 1821-1419 & 57372 & 6 & 109 & 7 & X & X & New - Our
measurement (bshaw)\tabularnewline
J1821-1419 & 1821-1419 & 58271 & 157 & X & X & X & X & New - Our
measurement (bshaw)\tabularnewline
B1822-09 & 1825-0935 & 58025 & 1 & 4.5 & 1 & X & X & New -
AGL\tabularnewline
B1822-09 & 1825-0935 & 58068 & 3 & X & X & X & X & New -
AGL\tabularnewline
B1822-09 & 1825-0935 & 58486.2 & 0.9 & 3.8 & 0.1 & X & X & New - AGL
(bshaw\_measurement)\tabularnewline
B1823-13 & 1826-1334 & 56556 & 4 & 2599 & 2 & 9 & 0.3 & New - Our
measurement\tabularnewline
B1823-13 & 1826-1334 & 58915 & 18 & 2486.2 & 0.4 & -6.37 & 0.08 & New -
bshaw/agl\tabularnewline
B1824-10 & 1827-0958 & 48764 & 6 & 0.4 & 0.1 & -0.2 & 0.3 & New - Our
measurement\tabularnewline
B1828-11 & 1830-1059 & 55041.75 & 0.04 & 6.2 & 0.1 & 5.2 & 0.2 & New -
Our measurement\tabularnewline
B1830-08 & 1833-0827 & 54782.2 & 0.1 & 0.55 & 0.02 & 0.27 & 0.05 & New -
Our measurement\tabularnewline
J1832+0029 & 1832+0029 & 53498 & 50 & 66 & 1 & 53 & 5 & New - cme (bshaw
values)\tabularnewline
B1834-10 & 1836-1008 & 55746.2 & 0.2 & 3.5 & 0.1 & 5.8 & 0.4 & New - Our
measurement\tabularnewline
J1835-1020 & 1835-1020 & 57590.6 & 0.3 & 3.29 & 0.01 & 2.3 & 0.3 & New -
Our measurement (bshaw)\tabularnewline
J1835-1106 & 1835-1106 & 58488 & 2 & 9.3 & 0.6 & 4 & 1 & New -
bshaw\tabularnewline
J1837-0604 & 1837-0604 & 55820 & 14 & 1395 & 3 & 5.9 & 0.1 & New - Our
measurement\tabularnewline
J1837-0604 & 1837-0604 & 56512 & 0.3 & 15.4 & 0.5 & 0.4 & 0.1 & New -
Our measurement\tabularnewline
J1837-0559 & 1837-0559 & 56223 & 6 & 0.6 & 0.1 & 0.7 & 0.1 & New - Our
measurement\tabularnewline
J1838-0453 & 1838-0453 & 58692 & 9 & 71 & 6 & -6 & 4 & New -
bshaw\tabularnewline
J1840-0221 & 1840-0221 & 55747 & 7 & 2.72 & 0.12 & 0 & 0 & New - Our
measurement (bshaw)\tabularnewline
J1841-0524 & 1841-0524 & 55524 & 19 & 805 & 1 & 0.79 & 0.03 & New - Our
measurement\tabularnewline
J1841-0524 & 1841-0524 & 56567.8 & 0.2 & 21.7 & 0.2 & 0.26 & 0.02 & New
- Our measurement\tabularnewline
J1841-0524 & 1841-0524 & 58978 & 140 & X & X & X & X & New - Awaiting
measurement\tabularnewline
B1841-04 & 1844-0433 & 49401 & 16 & 0.21 & 0.03 & 0.8 & 0.2 & New - Our
measurement\tabularnewline
J1841-0157 & 1841-0157 & 56921.4 & 0.1 & 32.78 & 0.01 & 2.9 & X & New -
Our measurement (bshaw)\tabularnewline
J1842+0257 & 1842+0257 & 57112 & 56 & 12060.9 & 0.2 & 1.3 & 0.3 & New -
Our measurement (bshaw/agl)\tabularnewline
J1844-0310 & 1844-0310 & 54410 & 4 & 1.8 & 0.2 & -0.5 & 0.2 & New - Our
measurement\tabularnewline
J1844+00 & 1844+00 & 56784.4 & 0.2 & 249.42 & 0.02 & 3.98 & 0.08 & New -
Our measurement (bshaw)\tabularnewline
B1844-04 & 1847-0402 & 55509 & 1 & 0.45 & 0.03 & 0.08 & 0.01 & New - Our
measurement\tabularnewline
B1844-04 & 1847-0402 & 56041 & 19 & 0.102 & 0.021 & 0 & 0 & New - Our
measurement (Shaw/Lyne)\tabularnewline
J1850-0026 & 1850-0026 & 56221.8 & 0.1 & 14.3 & 0.03 & 0.63 & 0.01 & New
- Our measurement\tabularnewline
J1850-0026 & 1850-0026 & 56425 & 11 & 92 & 0.1 & 0.39 & 0.04 & New - Our
measurement\tabularnewline
J1850-0026 & 1850-0026 & 57495.3 & 0.4 & 7.13 & 0.05 & 0.37 & 0.02 & New
- Our measurement (bshaw)\tabularnewline
J1850-0026 & 1850-0026 & 57708 & 9 & 1196.4 & 0.18 & 0.76 & 0.03 & New -
Our measurement (bshaw/agl)\tabularnewline
J1852-0026 & 1852-0026 & 54493 & 1 & 0.9 & 0.2 & -3 & 2 & new ? cme;
same as previous line? (I think this is just timing noise -
bshaw)\tabularnewline
J1853+0056 & 1853+0056 & 54981.7 & 0.4 & 5.1 & 0.4 & 3 & 1 & New - Our
measurement\tabularnewline
J1853+0056 & 1853+0056 & 54962.4 & 1.4 & 4.997 & 0.02 & 0.336 & 0.004 &
New - Our measurement (bshaw)\tabularnewline
B1853+01 & 1856+0113 & 57341 & 18 & 3843 & 1 & 5 & 0.2 & New - Our
measurement (bshaw/agl)\tabularnewline
J1854-1557 & 1854-1557 & 58632 & 35 & 8 & 7 & X & X & New -
AGL\tabularnewline
J1856+0245 & 1856+0245 & 56388 & 16 & 2672 & 5 & 7.9 & 0.2 & New - Our
measurement\tabularnewline
J1857+0143 & J1857+0143 & 58326 & 100 & X & X & X & X & New -
bshaw\tabularnewline
B1859+01 & 1901+0156 & 58188 & 41 & 4.3 & 0.1 & X & X & New -
bshaw\tabularnewline
B1900+06 & 1902+0615 & 55439.3 & 0.1 & 0.17 & 0.01 & 0.28 & 0.04 & New -
Our measurement\tabularnewline
J1901+0510 & 1901+0510 & 56260 & 80 & 143 & 10 & X & X & New - (agl) TOA
at 56257\tabularnewline
J1907+0631 & 1907+1631 & 56987.45 & 1 & 2105.5 & 0.4 & 5.14 & 0.07 & New
- Our measurement (bshaw)\tabularnewline
J1907+0631 & 1907+1631 & 57902.65 & 1 & 4977.6 & 0.5 & 4.3 & 0.04 & New
- Our measurement (bshaw)\tabularnewline
J1909+0749 & 1909+0749 & 57491 & 16 & 2844.4 & 0.4 & 3.82 & 0.05 & New -
Our measurement (bshaw/agl)\tabularnewline
J1909+0912 & 1909+0912 & 54988 & 1 & 4.8 & 0.3 & 0.1 & 0.1 & New - Our
measurement\tabularnewline
J1909+0912 & 1909+0912 & 57551 & 50 & 7400 & 100 & 12 & 1 & New - Our
measurement\tabularnewline
J1913+0446 & 1914+0446 & 55376.2 & 0.2 & 2 & 1 & 0 & 1 & New - Our
measurement\tabularnewline
J1913+0446 & 1913+0446 & 56574 & 1 & 1.5 & 0.1 & 0.04 & 0.02 & New - Our
measurement\tabularnewline
J1913+0904 & 1913+0904 & 56134.6 & 0.1 & 2.8 & 0.1 & 0.7 & 0.2 & New -
Our measurement\tabularnewline
J1913+1000 & 1913+1000 & 56601 & 10 & 487.9 & 0.4 & -5 & 1 & New - Our
measurement\tabularnewline
J1921+0812 & 1921+0812 & 55349 & 8 & 3633 & 0.1 & 5 & 1 & New - Our
measurement\tabularnewline
J1931+1817 & 1931+1817 & 58385.6 & 2 & 6.99 & 0.11 & 0.2 & 0.01 & New -
AGL\tabularnewline
J1931+1817 & J1931+1817 & 58392 & 3 & 8.4 & 0.5 & 0.5 & 0.1 & New - agl
(bshaw measurement)\tabularnewline
J1931+1817 & 1931+1817 & 58668 & 115 & X & X & X & X & New - bshaw
(unsure)\tabularnewline
B1946-25 & 1949-2524 & 50056 & 2 & 0.09 & 0.01 & 0.05 & 0.02 & New - Our
measurement\tabularnewline
B1951+32 & 1952+3252 & 55328 & 1 & 1500 & 1 & 28 & 1 & New (found by
Fermi people) - Our measurement\tabularnewline
J1957+2831 & 1957+2831 & 56903.695 & 0.002 & 2.2 & 0.1 & X & X & New -
Our measurement\tabularnewline
J2005-0020 & 2005-0020 & 55972.1 & 0.3 & 12.3 & 0.3 & 2 & 1 & New - Our
measurement\tabularnewline
J2021+3651 & 2021+3651 & 55110 & 1 & 2230 & 1 & 9.9 & 0.4 & New - Our
measurement\tabularnewline
J2021+3651 & 2021+3651 & 57204.89 & 0.02 & 3048 & 1 & 6.68 & 0.31 & New
- Our measurement (bshaw)\tabularnewline
B2020+28 & 2022+2854 & 47409 & 2 & 0.13 & 0.02 & 0.5 & 0.1 & New - Our
measurement\tabularnewline
B2021+51 & 2022+5154 & 58312 & 21 & 0.29 & 0.07 & X & X & New -
bshaw\tabularnewline
B2027+37 & 2029+3744 & 56993.7 & 0.1 & 6.21 & 0.19 & X & X & New - mjk
(bshaw values)\tabularnewline
J2032+4127 & 2032+4127 & 55821 & 13 & 276.2 & 0.5 & 0 & 1 & New - Our
measurement\tabularnewline
B2217+47 & 2219+4754 & 55859.43 & 0.05 & 1.14 & 0.01 & 1 & 0.1 & New -
Our measurement\tabularnewline
J2229+6114 & 2229+6114 & 55134 & 1 & 195 & 2 & 5.5 & 0.1 & New - Our
measurement\tabularnewline
J2229+6114 & 2229+6114 & 55601 & 2 & 1222 & 4 & 12.9 & 0.1 & New - Our
measurement\tabularnewline
J2229+6114 & 2229+6114 & 56366.59 & 0.02 & 65.9 & 0.2 & 3.32 & 0.02 &
New - Our measurement\tabularnewline
J2229+6114 & 2229+6114 & 57910 & 50 & 4 & X & X & X & New - Our
measurement (bshaw)\tabularnewline
J2229+6114 & 2229+6114 & 58423 & 7 & 1000 & X & X & X & New - Our
measurement (agl)\tabularnewline
1E\_2259+586 & 2301+5852 & 54040 & X & 11167 & X & X & X & Icdem+2012
{[}\textless a
href="http://adsabs.harvard.edu/abs/2012MNRAS.419.3109I"\textgreater ibi12\textless/a\textgreater{]}\tabularnewline
B2323+63 & J2325+6316 & 53998 & 46 & 0.24 & 0.01 & -0.2 & 0.03 & New -
Our measurement (bshaw)\tabularnewline
J2346-0609 & 2346-0609 & 57498 & 4 & 0.599 & 0.011 & 2.12 & 0.21 & New -
bshaw\tabularnewline
\bottomrule
\end{longtable}

==> table.tex <==
%\clearpage
%  79 LINES PER PAGE (OTHER THAN FIRST)
\begin{table}
  \begin{center}
%\caption{All glitches, previously published and found in this work. For re-analysed glitches the new values are shown, and the original references are given in the last column. Errors are given in parentheses on units  of the last quoted digit.Visit http://www.jb.man.ac.uk/pulsar/glitches.html for an online and up-to-date version of this Table.}
\caption{Table showing the measured glitch parameters from all of the new glitches in our sample. The first and the second columns list the J-name and the B-name of the pulsar. The third column indicates the glitch epoch and its uncertainty (in parentheses). The fourth and the fifth columns indicate the relative changes in the rotation frequency and its first order derivative. With the exception of the glitch epoch (see Appendix \ref{Apn1}, all uncertainties are quoted at the 2$-\sigma$ level.}
    \label{glitch_table}
    \begin{scriptsize}
    \begin{tabular}{lllll}
      \hline
      \hline
      \multicolumn{1}{c}{J-name}
      & \multicolumn{1}{c}{B-name}
      %& \multicolumn{1}{c}{No.}
      & \multicolumn{1}{c}{MJD} 
      & \multicolumn{1}{c}{$\Delta{\nu}/\nu$} 
      & \multicolumn{1}{c}{$\Delta{\dot{\nu}}/\dot{\nu}$} \\
      %& \multicolumn{1}{l}{References} \\
      \multicolumn{1}{c}{}
      & \multicolumn{1}{c}{}
      %& \multicolumn{1}{c}{Glt's}
      & \multicolumn{1}{c}{days}
      & \multicolumn{1}{c}{$10^{-9}$}
      & \multicolumn{1}{c}{$10^{-3}$}\\
      %& \multicolumn{1}{c}{} \\
      \hline 
      \hline 
%B Name   & J Name     & Epoch (MJD)   & $\frac{\Delta \nu}{\nu}$ & $\frac{\Delta \dot \nu}{\dot \nu}$ \\
J0157+6212 & B0154+61 & 58283(9)      & 2.6(3)                   & -                                 \\
J0205+6449 & -        & 54907(18)     & 1761(7)                  & 12(2)                              \\
J0205+6449 & -        & 55719(10)     & 126(5)                   & 3(1)                               \\
J0205+6449 & -        & 55836(5)      & 2933(5)                  & 13(1)                              \\
J0205+6449 & -        & 56854(28)     & 8(1)e+01                 & 3(2)                               \\[4.5pt]
J0205+6449 & -        & 57345(12)     & 527(7)                   & 5(1)                               \\
J0205+6449 & -        & 57696.8(2)    & 43(2)                    & -                                  \\
J0205+6449 & -        & 58320(97)     & 3140(5)                  & 20(3)                              \\
J0215+6218 & -        & 55900(37)     & 0.06(4)                  & -                                  \\
J0415+6954 & B0410+69 & 57040(23)     & 0.011(6)                 & -                                  \\[4.5pt]
J0417+35   & -        & 57053.6(2)    & 24.54(3)                 & 3.4(1)                             \\
J0525+1115 & B0523+11 & 56010(1)      & 0.312(2)                 & 0.6(2)                             \\
J0534+2200 & B0531+21 & 55875.49(3)   & 39(4)                    & 0.23(2)                            \\
J0534+2200 & B0531+21 & 57839.8(1)    & 2.2(4)                   & -                                  \\
J0534+2200 & B0531+21 & 58470.7(2)    & 2.3(6)                   & -                                  \\[4.5pt]
J0601-0527 & B0559-05 & 54362(56)     & 0.05(1)                  & -                                  \\
J0611+1436 & -        & 55818(16)     & 5575.4(8)                & -20(2)                             \\
J0625+1015 & -        & 55201(23)     & 0.33(5)                  & -                                  \\
J0625+1015 & -        & 57676(8)      & 1.17(6)                  & 0.9(2)                             \\
J0631+1036 & -        & 55119.3(2)    & 9.4(4)                   & -                                  \\[4.5pt]
J0631+1036 & -        & 55276.7(9)    & 7.5(6)                   & -                                  \\
J0631+1036 & -        & 55702(5)      & 3277.9(8)                & 2.7(6)                             \\
J0631+1036 & -        & 58341.7(3)    & 27.8(8)                  &                                    \\
J0631+1036 & -        & 58352.12(4)   & 96.4(6)                  & 1.3(3)                             \\
J0742-2822 & B0740-28 & 56725.2(7)    & 2.4(1)                   & -1.1(6)                            \\[4.5pt]
J0820-1350 & B0818-13 & 49925(58)     & 0.035(2)                 & 0.159(4)                           \\
J0820-1350 & B0818-13 & 58065(26)     & 0.082(6)                 & 0.14(7)                            \\
J0846-3533 & B0844-35 & 55682(17)     & 0.62(4)                  & 3(1)                               \\
J0922+0638 & B0919+06 & 55152(12)     & 1256.2(4)                & -                                  \\
J1635-2614 & -        & 56472(8)      & 0.71(3)                  & -                                  \\[4.5pt]
J1705-1906 & B1702-19 & 55170(9)      & 0.28(3)                  & -                                  \\
J1705-1906 & B1702-19 & 55956(5)      & 0.30(3)                  & -                                  \\
J1705-1906 & B1702-19 & 57957(31)     & 0.18(5)                  & -                                  \\
J1730-3350 & B1727-33 & 55908(30)     & 2254(1)                  & 5.3(5)                             \\
J1734-3333 & -        & 56339(12)     & 90(1)                    & -                                  \\[4.5pt]
J1740-3015 & B1737-30 & 55213(75)     & 2663(3)                  & 1.2(3)                             \\
J1740-3015 & B1737-30 & 55936.4(5)    & 18.3(6)                  & 0.4(2)                             \\
J1740-3015 & B1737-30 & 57468.60(1)   & 229.4(4)                 & 1.2(4)                             \\
J1740-3015 & B1737-30 & 58241(8)      & 837.9(7)                 & 2.0(3)                             \\
J1737-3102 & -        & 57087(4)      & 18(1)                    & -                                  \\[4.5pt]
J1737-3137 & -        & 57115(9)      & 7.0(7)                   & -                                  \\
J1737-3137 & -        & 58147(42)     & 4498(1)                  & 1.3(1)                             \\
J1740+1000 & -        & 56164(10)     & 2910.9(4)                & 11(1)                              \\
J1746-2856 & -        & 57038(4)      & 24.4(4)                  & 2.1(3)                             \\
J1751-3323 & -        & 57019(3)      & 13(1)                    & -5(2)                              \\[4.5pt]
J1757-2421 & B1754-24 & 55716(21)     & 7807(1)                  & 6.3(5)                             \\
J1801-2451 & B1757-24 & 56979(36)     & 2413(4)                  & 5.3(8)                             \\
J1801-2304 & B1758-23 & 55361(7)      & 2.9(7)                   & -                                  \\
J1801-2304 & B1758-23 & 55836(12)     & 1.7(5)                   & -                                  \\
J1801-2304 & B1758-23 & 56149.02(2)   & 513.8(4)                 & 1.2(7)                             \\[4.5pt]
J1801-2304 & B1758-23 & 57586.3(4)    & 96.6(9)                  & -                                  \\
J1809-2004 & -        & 56227.6(6)    & 48.67(5)                 & 0.79(3)                            \\
J1814-1744 & -        & 55625(8)      & 16(4)                    & 0.3(2)                             \\
J1827-0958 & B1824-10 & 48762(65)     & 0.4(1)                   & -                                  \\
J1835-1020 & -        & 57590(1)      & 3.26(2)                  & 0.2(1)                             \\[4.5pt]
J1826-1334 & B1823-13 & 56556(7)      & 2599.7(3)                & 10.1(4)                            \\
J1830-1059 & B1828-11 & 55040.9(5)    & 6.3(5)                   & -                                  \\

\hline \multicolumn{7}{r}{{\dots \sl continued on next page}}\\
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}

\begin{table}
  \begin{center}
    \begin{scriptsize}
    \contcaption{}
    \begin{tabular}{lllll}
      \hline
      \hline
      \multicolumn{1}{c}{J-name}
      & \multicolumn{1}{c}{B-name}
      %& \multicolumn{1}{c}{No.}
      & \multicolumn{1}{c}{MJD} 
      & \multicolumn{1}{c}{$\Delta{\nu}/\nu$} 
      & \multicolumn{1}{c}{$\Delta{\dot{\nu}}/\dot{\nu}$} \\
      %& \multicolumn{1}{l}{References} 
      \multicolumn{1}{c}{}
      & \multicolumn{1}{c}{}
      %& \multicolumn{1}{c}{Glt's}
      & \multicolumn{1}{c}{days}
      & \multicolumn{1}{c}{$10^{-9}$}
      & \multicolumn{1}{c}{$10^{-3}$}\\
     % & \multicolumn{1}{c}{} \\
      \hline \hline
J1833-0827 & B1830-08 & 54778(6)      & 0.5(1)                   & 0.15(8)                            \\
J1836-1008 & B1834-10 & 55744.5(9)    & 3.6(1)                   & -                                  \\
J1837-0604 & -        & 55821(23)     & 1398(1)                  & 6.9(7)                             \\[4.5pt]
J1837-0604 & -        & 56511(1)      & 16.7(8)                  & -                                  \\
J1837-0559 & -        & 56340(23)     & 0.2(2)                   & -                                  \\
J1837-0559 & -        & 58022(12)     & 3.4(3)                   & -                                  \\
J1839-0223 & -        & 56994(5)      & 3.17(4)                  & 3.5(2)                             \\
J1841-0524 & -        & 55525(35)     & 804.9(4)                 & 0.8(1)                             \\[4.5pt]
J1841-0524 & -        & 56565(2)      & 21.6(4)                  & -                                  \\
J1844-0433 & B1841-04 & 49355(28)     & 0.22(1)                  & -0.03(2)                           \\
J1841-0157 & -        & 56924(1)      & 33.3(4)                  & -                                  \\
J1842+0257 & -        & 57112(55)     & 12060.9(2)               & 1.0(3)                             \\
J1844+00   & -        & 56784(43)     & 249.55(3)                & 4.1(7)                             \\[4.5pt]
J1845-0743 & -        & 57943(65)     & 0.04(1)                  & -0.11(9)                           \\
J1847-0402 & B1844-04 & 55502(7)      & 0.52(4)                  & 0.04(3)                            \\
J1849-0317 & -        & 58306(12)     & 33(2)                    & -                                  \\
J1850-0026 & -        & 56239(2)      & 14.2(3)                  & 0.9(2)                             \\
J1850-0026 & -        & 56425(11)     & 91.9(3)                  & 0.8(2)                             \\[4.5pt]
J1850-0026 & -        & 57495(2)      & 7.0(2)                   & 0.7(2)                             \\
J1850-0026 & -        & 57708(9)      & 1196.7(2)                & 0.8(2)                             \\
J1853+0056 & -        & 54970(4)      & 5.4(1)                   & 0.4(1)                             \\
J1856+0113 & B1853+01 & 57325(34)     & 3489(4)                  & 2.8(9)                             \\
J1856+0245 & -        & 56388(16)     & 2672.5(7)                & 8.4(3)                             \\[4.5pt]
J1901+0156 & B1859+01 & 58149(40)     & 1053.02(6)               & 2.1(4)                             \\
J1902+0615 & B1900+06 & 55436(16)     & 0.19(3)                  & -                                  \\
J1907+0631 & -        & 56987(8)      & 2106(2)                  & 5.0(5)                             \\
J1907+0631 & -        & 57901(54)     & 4986(5)                  & 4.7(7)                             \\
J1909+0749 & -        & 57492(16)     & 2904.2(9)                & 3.7(2)                             \\[4.5pt]
J1909+0912 & -        & 54980(1)      & 4.4(3)                   & 0.09(8)                            \\
J1909+0912 & -        & 57552(60)     & 7389.8(3)                & 4.58(9)                            \\
J1913+0446 & -        & 55368(3)      & 2.5(2)                   & -                                  \\
J1913+0446 & -        & 56549(14)     & 0.8(2)                   & 0.2(1)                             \\
J1913+0904 & -        & 56132.8(6)    & 3.2(2)                   & -                                  \\[4.5pt]
J1913+1000 & -        & 56600(1)      & 491(1)                   & -                                  \\
J1921+0812 & -        & 55367(33)     & 3632.9(1)                & 3.0(7)                             \\
J1952+3252 & B1951+32 & 55328(3)      & 1489.9(4)                & 5.4(4)                             \\
J1957+2831 & -        & 56897(2)      & 2.25(6)                  & 1.3(5)                             \\
J2005-0020 & -        & 55976(5)      & 12.5(6)                  & -                                  \\[4.5pt]
J2021+3651 & -        & 55110(2)      & 2228.8(9)                & 8.5(7)                             \\
J2021+3651 & -        & 57200(8)      & 3069(2)                  & 10.2(9)                            \\
J2029+3744 & B2027+37 & 56993(2)      & 6.2(2)                   &                                    \\
J2032+4127 & -        & 55820(9)      & 273.3(1)                 & 1.06(4)                            \\
J2219+4754 & B2217+47 & 55857(1)      & 1.16(2)                  & 0.4(3)                             \\[4.5pt]
J2229+6114 & -        & 55134(2)      & 198.4(6)                 & 6.3(4)                             \\
J2229+6114 & -        & 55601(4)      & 1223.6(6)                & 13.0(5)                            \\
J2229+6114 & -        & 56362(5)      & 66.0(9)                  & 3.2(5)                             \\
J2229+6114 & -        & 58424(6)      & 1047.1(9)                & 12.4(6)                            \\
J2325+6316 & B2323+63 & 53948(85)     & 0.21(2)                  & -0.32(4)                           \\[4.5pt]
J2346-0609 & -        & 57495(7)      & 0.55(1)                  & 2.4(4)                           \\
\hline \hline
\end{tabular}
\end{scriptsize}
\end{center}
\end{table}
